FairTest: Discovering Unwarranted Associations in Data-Driven Applications

In a world where traditional notions of privacy are increasingly challenged by the myriad companies that collect and analyze our data, it is important that decision-making entities are held accountable for unfair treatments arising from irresponsible data usage. Unfortunately, a lack of appropriate methodologies and tools means that even identifying unfair or discriminatory effects can be a challenge in practice. We introduce the unwarranted associations (UA) framework, a principled methodology for the discovery of unfair, discriminatory, or offensive user treatment in data-driven applications. The UA framework unifies and rationalizes a number of prior attempts at formalizing algorithmic fairness. It uniquely combines multiple investigative primitives and fairness metrics with broad applicability, granular exploration of unfair treatment in user subgroups, and incorporation of natural notions of utility that may account for observed disparities. We instantiate the UA framework in FairTest, the first comprehensive tool that helps developers check data-driven applications for unfair user treatment. It enables scalable and statistically rigorous investigation of associations between application outcomes (such as prices or premiums) and sensitive user attributes (such as race or gender). Furthermore, FairTest provides debugging capabilities that let programmers rule out potential confounders for observed unfair effects. We report on use of FairTest to investigate and in some cases address disparate impact, offensive labeling, and uneven rates of algorithmic error in four data-driven applications. As examples, our results reveal subtle biases against older populations in the distribution of error in a predictive health application and offensive racial labeling in an image tagger.

==> Makefile <==
PAPER=paper
LATEX=pdflatex

BIBTEX=bibtex

SRCS=$(wildcard *.tex)
REFS=$(wildcard *.bib)
FIGS=$(wildcard figures/*)

.PHONY: results $(PAPER).pdf clean

all: $(PAPER).pdf

$(PAPER).pdf: $(SRCS) $(REFS) $(FIGS)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)


submission: $(PAPER).pdf
	cp $(PAPER).pdf submission/

clean:
	rm -f *.dvi *.aux *.log *.blg *.out *.synctex.gz \
          $(PAPER).ps $(PAPER).pdf \
          $(PAPER)-single.pdf $(PAPER)-single.ps


==> applications.tex <==
\subsection{Applications and Datasets}
\label{sec:investigations:applications}

To experiment with \sysname, we assembled a diverse set of microbenchmarks,
real datasets, simulations, and real applications, which we used to perform
various investigations or to evaluate various properties of \sysname
(see \S\ref{sec:evaluation}).
Our goal was to exercise \sysname as much as possible to identify its
strengths and weaknesses.
Our set, which we plan to release as a benchmarking suite for future
algorithmic fairness works, includes seven workloads:

\begin{itemize}

\item {\em One tightly controlled microbenchmark}, which we use to evaluate
when \sysname's bug detection abilities when we know ground truth for the
associations;

\item {\em Two well-known datasets} (the \emph{Adult Census} dataset from the
UCI ML-repository~\cite{uci_repo} and the 1973 Berkeley
Admissions~\cite{bickel75}), which have been used in prior algorithmic fairness
literature and which we use to confirm that \sysname can detect known
disparate-impact effects (and in some cases discover previously unknown ones);
and

\item {\em Four data-driven applications} that we feed with real data:
(1) a simulator of Staples's pricing engine (as described by the WSJ
report~\cite{staples}) fed by U.S. census data, (2) a movie recommender
system based on the Apache Mahout recommendation engine and fed by the
popular MovieLens dataset~\cite{movielens}, (3) a predictive healthcare
application, the winner of the 2012 Heritage Health Prize Competition for
predictive medicine, fed by the dataset released as part of that competition,
and (4) an image tagging system based on the OverFeat network~\cite{overfeat},
fed by images of people from the popular ImageNet dataset~\cite{imagenet}.

\end{itemize}

Table~\ref{tab:applications} summarizes various relevant statistics,
such as the number of users and of sensitive features, plus the types of
investigations we ran for each, and the metrics we used.
In subsequent sections, we will detail these applications and datasets as
needed by the specific experiment.

\heading{Controlled Microbenchmark.}
For the specific purpose of \sysname evaluation, we created a microbenchmark
that lets us control the strength and span of association bugs.
With it, we evaluate \sysname's ability to discover various types of bugs,
as well as its discovery limits.
We use U.S Census~\footnote{\url{http://www.census.gov}} demographics for
gender, race and income to generate 1 million synthetic users.
We create an initially ``fair'' algorithm that randomly provides each user
with output $A$ or $B$.
We then artificially induce disparities in certain sub-populations as follows.
In a few states, we provide users of a particular race with output $A$ with
probability $(\frac12\pm \Delta)$, depending on their income.
For various sub-population sizes and values of $\Delta$, we inject 10 random
discrimination contexts into our data, and check how many \sysname discovers
as a function of the effect's strength.

\heading{Staples Simulation.}
We created a simulation of Staples' scheme
we simulate Staples' scheme and use \sysname to test
for price disparities across different ethnic groups or income levels. Our dataset consists of 1 million synthetic users (generated using the U.S.
census demographic information for
income, gender, and ethnic groups) along with a price presented
to these users by our algorithm.
To set prices, we collect store locations of HomeDepot, a competitor brick-and-mortar store, and offer discounted prices to all users living in a 20 miles radius of these stores~\cite{staples}.

\heading{Predictive Healthcare Application.}
The goal of the \emph{Heritage Health Prize Competition}~\footnote{\url{http://www.heritagehealthprize.com}} was to ``develop a breakthrough algorithm that uses available patient data to predict and prevent unnecessary hospitalizations [and] could be used by health care providers [to] develop new care plans and strategies''.
Using the methods of the team `Market Makers', winners of the competition's first two milestones, we build an application predicting hospital visits, given historical patient claims. We consider two variants of this problem, (1) as a regression task as in the original competition (how many days will a user stay in the hospital?) and (2) as a simpler binary task (will a user stay in the hospital?).
For both tasks, we use $25\%$ of the available data ($28785$ users) to train a gradient-boosted random forest, that we then apply to the remaining data. We achieve $85\%$ accuracy for binary classification and a root-mean-squared-log error of $0.4$ for regression.

\heading{Movie Recommender.}
We use 1 million ratings (on a 1-5 scale) of 3,900 movies made by 6,040
MovieLens users~\cite{movielens} to implement a movie
recommendation application. MovieLens users are tagged with demographic
information, such as age and gender; movies are similarly tagged with metadata, such as publish date and genre (e.g., drama, action).
We train a recommender using the ALS algorithm~\cite{matrixFactor} and generate 50 recommendations for new movies, based on user's personal preferences.

\heading{Image Tagger.}
We collect $1405$ images of black people and $1243$ images of white people from
the ImageNet database~\cite{imagenet}, and output 5 labels per
image using the OverFeat network~\cite{overfeat}. This image tagger was
trained on $1000$ ImageNet categories, mainly animals and
everyday objects but \emph{not} images of
people. Consequently, by applying it to the images we collected, we are
evaluating how an \emph{under-trained} algorithm may associate labels
with different groups of users. Interestingly, Google's image tagging bug has raised the question of whether such bugs were due, in part, to an under-representation of certain ethnic groups in tech companies~\cite{googleGorilla}.

\heading{Existing Datasets.}
We also apply \sysname to two historically famous datasets, the \emph{1973 Berkeley
admission data}~\cite{bickel75} and the \emph{Adult Census}
dataset from the UCI ML-repository~\cite{uci_repo}. The Berkeley dataset is used to illustrate how a developer may (1) use \sysname to automatically discover
instances of Simpson's paradox or (2) specify an \emph{explanatory feature} that
accounts for an observed bias.
The Adult Census data differs from other datasets we consider, in that the `outcome' (a user's income) is not linked to a particular `decision' -- whether human or automated-- but rather to a complex mixture of individual and societal factors. We use
this dataset to show how \sysname's methods extend to a broader range of
applications than just data-driven algorithms, such as for uncovering contexts
of \emph{social bias} -- in this case differences in income levels across genders and ethnic groups.



==> effect-sizes-ranking.tex <==
% !TEX root = paper.tex

% \subsection{Ranking and Filtering Association Bugs Module}
% \label{sec:design:rank_filter}

%We note that ranking bugs by their p-values does not provide the same properties: a small effect on a
%large subpopulation may have a smaller p-value than one with a
%considerably larger effect on a smaller subpopulation (see \F\ref{fig:adult-bug-report}).
% Note (Ari): I removed remark that we considered ranking by p-values, as this is an incorrect methodology

\iffalse
In addition to these post-hoc rules for filtering and ranking, we
proactively filter for {\em obviously explained or necessary associations}.
A programmer may specify a set of {\em explanatory features}, or
properties of a user on which it is deemed acceptable to
differentiate.
For example, a company may decide that giving discounts to loyal
customers is always admissible even if it leads to a pricing bias against
groups of less avid customers.
Explanatory features can also encode the notion of {\em
business necessity} supported by discrimination law, which justifies
disparate effects given certain imperative business requirements~\cite{ruggieri10}.
% Ari: Business necessity generally refers to employment decisions, so I removed the indication that it's a general notion

\sysname lets developers declare user
% It's technically not the filtering mechanism that does this, as we need to know E already suring
% the tree construction, to avoid looking for explainable contexts
features $\EA$ as necessary/explanatory for the application and
explicitly avoids deriving associations that are accounted for by
these features. To this end, it uses modified association
metrics that measure the dependence of protected features $\PA$ and outputs
$\OUT$ \emph{conditioned} on $\EA$ (\eg \emph{conditional mutual
information} $I(\PA;\OUT|\EA)$).

In addition to supporting business necessity and obvious explanations,
explanatory features have another, compelling feature for \sysname:
they enable {\em debugging} by letting developers eliminate plausible causes
for association bugs.
We have leveraged this feature in our investigations and will
demonstrate its value in \S\ref{sec:investigations}.
\fi

\iffalse
A more effective filtering additionally takes into account the tree
structure formed by the different discrimination contexts: display a node
only if it exhibits a larger bias (as measured by the effect size
described above) than all of its parents.
This lets a developer track how the disparate impact of an algorithm's
unwarranted associations increases in more and more specific user
subpopulations.
\fi


\iffalse
\sysname filters and ranks association bugs to allow developers to efficiently identify those subpopulations that appear most affected by an algorithm's behavior.
Bugs are ranked by their \emph{effect-size}, specifically by the lower-end of the confidence interval computed for each context. This ranking prioritizes populations that appear most affected by an unwarranted association, but also lets us report weak effects that are nevertheless statistically significant because they affect very large populations. Ranking bugs by their p-values, which we considered but rejected, does not share this property: a low effect over a large population may be statistically more significant than a considerably larger effect in a smaller context.

In addition to filtering-out contexts with a statistically insignificant effect (for a chosen false discovery rate), \sysname uses a more elaborate filtering scheme that takes into account the tree structure formed by the discovered association contexts. We report a context only if it exhibits a larger association (as measured by the effect size described above) than all of its parents. A developer can thus efficiently track how the impact of an algorithm's unwarranted associations increases in more and more specific user subpopulations.
Note that our approach avoids fixing a manual threshold for what constitutes a notable effect. Instead, \sysname enables the discovery of a wide spectrum of bugs, ranging from strong associations that affect small population niches, to weaker effects that broadly affect a large subset of the users.

\fi


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Today's applications and web services collect and mine vast quantities of
personal information: clicks, locations, visited websites, social
interactions, and more.
Personal data offers great opportunities to improve personal, business,
and societal effectiveness.
It can boost applications' utility by personalizing their features, contents,
and recommendations; increase business revenues via targeted product
placement; and improve a wide range of social processes, such as healthcare,
disaster response and crime prevention.

Despite these benefits, integrating user data into applications
can have unintended and detrimental consequences -- such as the unfair
treatment of users -- that are difficult for developers to anticipate.
A case in point is the Staples differential pricing case~\cite{staples}:
Staples' seemingly rational decision to adjust online prices based on user
proximity to competitor brick-and-mortar stores led to higher prices for
low-income customers, who (as it turns out) generally live farther from these
stores.
Staples' intentions aside, this case underscores the difficulty of
foreseeing all the subtle implications and risks of data-driven heuristics.
And these risks will only increase as new kinds of personal data -- \eg
collected through the Internet of Things -- pass through increasingly complex
machine learning (ML) algorithms, with associations and inferences that may be
impossible to foresee.

It is no wonder, then, that reports of discriminatory effects in data-driven
applications litter the news.
Google's image tagger was recently found to associate racially offensive
labels with images of black people~\cite{googleGorilla}.
Discriminatory online advertising has been shown to associate ads for
lower-paying jobs with women~\cite{adFisher} and offensive, racially charged
ads with black people~\cite{sweeney13}.

Undesirable algorithmic biases often affect recognized, vulnerable
subpopulations (defined by race, gender, age, etc.), but can affect other
subpopulations, as well.
We thus refer broadly to such biases as {\em unwarranted associations}.
We argue that unwarranted associations are new kinds of {\em bugs} specific to
modern, data-driven applications, which programmers have a duty to proactively
check for, debug, and fix with the same urgency as they apply to other
security and privacy bugs.
Unwarranted associations may offend and even harm users, and cause programmers
and businesses embarrassment, mistrust, and potentially loss of revenue.
Unwarranted associations may also be symptoms of a malfunction of a
data-driven algorithm, such as a ML algorithm exhibiting poor
accuracy for minority groups that are under-represented in its training
set~\cite{hardt14}.

\input{introduction-common}

==> prototype.tex <==

\section{Prototypes and Deployment}

We implemented \sysname in Python, to be used as a
standalone library or as a RESTful service.
As a library, our prototype's workflows are designed to integrate
with Pandas, SciPy's popular data analysis library, allowing developers to incorporate \sysname into their typical
application testing process.
Our service prototype enables continuous monitoring for association
bugs in production systems.
Developers register investigations with the \sysname service and route
user attributes and outputs to it.
\sysname runs investigations periodically and sends reports to the
developers.
The monitoring service continuously collects new data to
replenish its test sets, thereby supporting larger numbers of
investigations than the standalone library running on static datasets.
% All code will be released upon publication.


\iffalse
A key question is where programmers can obtain the data required to
analyze their applications with \sysname.
Generally, we believe developers should use whatever relevant user data is available (which could include gender, race, location) and feed it into
\sysname as protected or contextual attributes.
Programmers can also use public datasets to emulate realistic application
users (as we do for Staples, see\sec\ref{sec:report-example}).
Finally, although not yet implemented, we envision a
deployment model where a separate, trusted entity (such as the EFF
or a census organization) collects a wider variety of user attributes,
and offers the \sysname RESTful service to a range of privacy-conscious
programmers interested in inspecting their applications for unwarranted
associations.
\fi

==> relwork.tex <==

\section{Related Work}
\label{sec:relwork}

We addressed some related works in\sec\ref{sec:motivation:candidate-approaches}.
Because our work is inter-disciplinary, drawing from both privacy and
ML, we detail specific works to give more context to people from different
communities.

\heading{Algorithmic Fairness.}
Our work is most closely related to the growing field of \emph{algorithmic fairness},
initiated by the work of Pedreschi et al.~\cite{pedreschi08}. Their notion of
fairness, based on manually imposed thresholds for binary association metrics,
has been adopted many other works on discrimination
detection~\cite{ruggieri10,ruggieri10a,feldman14,zliobaite11,luong11} and
prevention~\cite{kamiran09,kamiran10,calders10,feldman14,zliobaite11,luong11,hajian13}.
Some have defined fairness using binary metrics (\eg
\emph{a-protection}~\cite{ruggieri10, ruggieri10a, hajian13},
\emph{e-fairness}~\cite{feldman14}), although a few works also consider more
general association measures that are more broadly applicable (\eg
\cite{zemel13,kamishima12}).

\iffalse

A sizeable literature on {\em algorithmic fairness} has focused
on techniques for both {\em preventing} and {\em detecting} unfairness
in machine learning and data mining algorithms.
Existing work, however, provides neither tools that meet
our preceding requirements nor adequate foundations to create them.
Work on unfairness detection has focused on
testing for specific discrimination bugs akin to those in
Example 2; only one recent work~\cite{adFisher} addresses
discovery of such bugs (Example 1) in a very specific, ad-oriented
setting; error profiling (Example 3) has never been considered.
More importantly, our review has revealed important
limitations in definitional foundations and in the development and evaluation
of usable tools for data-driven programmers.

We closely studied 14 representative works from the algorithmic fairness
field: seven on discrimination prevention~\cite{kamiran09,kamiran10,calders10,
kamishima12,dwork12,zemel13,hajian13}, four on discrimination detection~\cite{pedreschi08,ruggieri10,ruggieri10a,adFisher}, and three on
both~\cite{feldman14,zliobaite11,luong11}.
We make four observations about the field's state.


\noindent
$\bullet$ {\em No generic, broadly-applicable system design:}
The range of fairness criteria proposed in the literature is
large and fragmented.
It includes: ratio proportions and
differences~\cite{pedreschi08, kamiran09,kamiran10,calders10,
ruggieri10, ruggieri10a, luong11, zliobaite11, hajian13, feldman14},
a-protection~\cite{ruggieri10, ruggieri10a, hajian13},
e-fairness~\cite{feldman14}, statistical parity~\cite{dwork12,
zemel13} and mutual information~\cite{kamishima12}.
All these criteria measure some form of association of program {\em
outputs} (\eg prices, errors) on {\em
protected user attributes} (\eg race, gender).
Our analysis of these criteria suggests that each metric is best suited for specific situations and data types, and there is no best criterion for all use cases.
Yet, each proposed unfairness detection or prevention mechanism tends to apply only to specific metrics that cover a limited range of cases. For instance, the majority of prior works only consider
binary protected features and outputs~\cite{pedreschi08,
kamiran09,kamiran10,calders10, ruggieri10, ruggieri10a, luong11,
zliobaite11, hajian13, feldman14}.
In this paper, we thus
{\em integrate multiple,
carefully chosen fairness criteria into a coherent system design with
broad applicability}.

\noindent
$\bullet$ {\em Limited consideration of discrimination contexts:}
Most prior work~\cite{kamiran09, kamiran10, calders10, zliobaite11, kamishima12, feldman14}
considers algorithmic fairness
solely at full user population level.
Yet it has been shown that discriminatory effects in a population
may differ from, and even contradict, those exhibited in
smaller subsets, an effect known as Simpson's paradox~\cite{simpson51}.
A famous example is the Berkeley admissions data~\cite{bickel75}:
University-wide admission rates appeared to disfavor women, yet when looking for similar
effects in each department, either no bias or an inverse bias
was found, because women tended to apply to departments with lower acceptance rates.
%The cause of this counter-intuitive effect was that women tended to apply to
%departments with lower acceptance rates.
%Unfortunately, the majority of prior works do not consider discrimination
%contexts as part of their system designs.
The few existing methods for discovering discrimination contexts~\cite{ruggieri10, ruggieri10a, luong11}
exhaustively assess all population subsets, leading to a number of
contexts that is exponential in the feature space~\cite{ruggieri10, ruggieri10a}
or linear in the user space~\cite{luong11}.
These works further fail to account for multiple-hypothesis testing for the many contexts they
consider, raising concerns about the statistical validity of their results.
In our work, we develop a method for {\em efficiently and rigorously
identifying meaningful discrimination contexts}.

\noindent
$\bullet$ {\em Relying on effect-size thresholds rather than statistical significance:}
Most prior algorithmic fairness work defines fairness based on manually selected thresholds, \ie   an algorithm is considered fair if a
chosen bias metric falls below a threshold.
Setting thresholds appears difficult (practically and morally) as it implies fixing a {\em permissible level} of
discrimination~\cite{peresie09}.
In fact, in legal practice, it is customary to consider the
\emph{statistical significance} of a discriminatory effect in addition to a measure
of that effect.
For instance, in U.S. hiring law, a ratio of 4/5 for the hiring rates of two groups is generally considered discriminatory, but lower effects may also qualify
if statistically significant (and higher effects may be ignored
if statistically insignificant)~\cite{ugesp78}.
Some authors have included confidence intervals for fairness metrics; these incorporate a notion
of statistical significance, but the authors persisted in defining fairness strictly
in terms of fixed thresholds on the effect size, sacrificing the opportunity of
detecting weak effects that occur in larger populations (i.e., subtle but
systematic discrimination).
%In addition, works that have reasoned about an algorithm's behavior in various subpopulations~\cite{ruggieri10, ruggieri10a, luong11} have failed to correct
%effect sizes to account for multiple comparisons and thus provide only weak guarantees on the false positive rate of their discoveries.
In contrast, our method {\em rigorously and comprehensively
detects any statistically significant discrimination cases, and ranks these
cases by their effect sizes}.

\noindent
$\bullet$ {\em Limited experimentation:}
\fi

Most prior work describes limited
experimental results, usually in the context of two datasets or less~\cite{calders10, kamiran09, kamiran10, ruggieri10, ruggieri10a, zliobaite11, kamishima12, dwork12, hajian13}.
We believe that extensive experience with many applications and datasets is
crucial for developing a robust and flexible system, one that can address real-world algorithmic fairness issues. Prior research also fails to cover system design issues, such as scalability and usability for developers.
In our work, we conduct
{\em an extensive experimental evaluation of \sysname
with six real-world applications and datasets}.

Most prior works assess fairness at the full user population level, but do not
consider discrimination manifesting in subpopulations~\cite{kamiran09,
kamiran10, calders10, zliobaite11, kamishima12, feldman14}. Works that do
integrate a notion of discrimination context~\cite{ruggieri10, ruggieri10a,
luong11} essentially resort to exhaustive enumeration of subpopulations, which
is not scalable and is prone to overfit (as they fail to correct for multiple
testing).  Prior works also largely ignore plausible explanations for
associations~\cite{feldman14,luong11,kamiran09,kamiran10,calders10, hajian13,
kamishima12}.

Finally, a line of work initiated by Dwork et al.~\cite{dwork12, zemel13} has
considered fairness from an \emph{individual's} point of
view, essentially aiming at building classifiers that \emph{treat similar
people similarly}.
A fundamental issue with this approach is that fairness is
defined with respect to a socially agreed-upon \emph{similarity
metric} for users in a given context~\cite{dwork12}.
Constructing this metric is non-trivial, especially using
only information about individuals in a small sample, as
opposed to \emph{every individual from the population}.
It is also non-trivial to test proposed notion of fairness on
a sample~\cite{jha2013testing,dixit2013testing}.

\heading{Web Transparency.}
Our work also relates to the emerging field of {\it web
transparency}~\cite{Hannak:2013uk,Xing:2014ws,Hannak:2014do,Vissers:2014uo,
Barford:2014ug,BinLiu:2013jn,Book:2015ue,adFisher,Lecuyer:2014wj,LSSCGH15-sunlight}.
Although some works touch on discrimination
and fairness (e.g.,~\cite{adFisher}), their setting is different: These works rely on {\em controlled, randomized experiments} that {\em probe} a service
with different inputs (generally not real user profiles) and observe the effects on outputs,
so as to identify and quantify Web services' use of personal data to target,
personalize, and tune prices.
Detection of unfair or unwarranted associations, as in \sysname, requires making
inferences from application behavior on {\em real user profiles}, which may
contain attribute correlations that do not
manifest in fabricated user profiles.

\heading{Debugging Machine Learning Applications.}
%This header can mean at least two different things.
%The first are techniques to ensure a correct implementation of a
%well-specified learning algorithm (\eg a gradient descent algorithm
%for a particular objective function).
%The second are techniques to improve modeling and/or predictive
%performance of a classifier or predictor learned on training data.
%Here, we are primarily concerned with this second notion of debugging,
%although incorrect implementations of well-specified algorithms may
%also be diagnosed with similar techniques.
ML practitioners often use exploratory data analysis
tools to understand data features and modeling errors~\cite{ng2011advice,ng2013error,hastie2009elements}.
This includes conducting ablative analyses, examining feature
dependency plots, and identifying commonalities among error cases.
These techniques are insufficient for unwarranted association discovery,
as shown in \S\ref{sec:motivation:candidate-approaches}.

Certain learning algorithms are directly amenable to post-learning
introspection.
For example, some works~\cite{kabra2015understanding} use bootstrap
resampling to assess the influence of a single training example.
In general, this is computationally prohibitive, but they provide a fast
approximation tailored to boosting~\cite{freund1997decision}.
Yet other methods, like Random Forests~\cite{breiman2001random,breiman2002wald},
produce classifiers that more amenable to introspection.
%Other works~\cite{breiman2002wald} show that when using Random
%Forests~\cite{breiman2001random}, the practitioner can ``[look] inside
%the black box'' (i.e., inspect the learned predictor) to perform
%introspective analyses such as assessing the effects of features,
%clustering of training examples, and identification of outliers.
Using these methods in \sysname instead of the guided decision tree
algorithm we developed would require similar adaptation for the goal
of detecting unwarranted associations.

